On the Local Communication Complexity of Counting and Modular Arithmetic

In standard number-in-hand multi-party communication complexity, performance is measured as the total number of bits transmitted globally in the network. In this paper, we study a variation called local communication complexity in which performance instead measures the maximum number of bits sent or received at any one player. We focus on a simple model where $n$ players, each with one input bit, execute a protocol by exchanging messages to compute a function on the $n$ input bits. We ask what can and cannot be solved with a small local communication complexity in this setting. We begin by establishing a non-trivial lower bound on the local complexity for a specific function by proving that counting the number of $1$'s among the first $17$ input bits distributed among the participants requires a local complexity strictly greater than $1$. We further investigate whether harder counting problems of this type can yield stronger lower bounds, providing a largely negative answer by showing that constant local complexity is sufficient to count the number $1$ bits over the entire input, and therefore compute any symmetric function. In addition to counting, we show that both sorting and searching can be computed in constant local complexity. We then use the counting solution as a subroutine to demonstrate that constant local complexity is also sufficient to compute many standard modular arithmetic operations on two operands, including: comparisons, addition, subtraction, multiplication, division, and exponentiation. Finally we establish that function $GCD(x,y)$ where $x$ and $y$ are in the range $[1,n]$ has local complexity of $O(1)$. Our work highlights both new techniques for proving lower bounds on this metric and the power of even a small amount of local communication.

==> circuit.tex <==
\section{Connections to Circuit Complexity}

We begin by showing how to simulate linear sized circuits with protocols in our model that require
only constant local complexity.

The below theorem establishes that a circuit of size $cn$, for constant $c> 1$,
can be simulated by $n$ players in our model with a local complexity bounded by $9c$.
The proof begins by transforming the circuit into an equivalent circuit with bounded
fan-out. The new circuit is at most only a constant factor larger than the original.
It then constructs an ordering on the gates that ensures that gates providing
the input for a given target gate $t$ show up before $t$ in the ordering.
Our protocol has each player simulate a constant number of gates from the circuit.
They use this ordering to specify a token-passing schedule that allows them to
compute their simulated gates' outputs, and then communicate this information to the
gates where it arrives as input, with a minimal local complexity.
%The details of this strategy are in the appendix.

Before moving on to our main theorem proof,
we must first specify our assumptions about the gates used in these circuits.
In the following results, we assume the standard gate definitions for the circuits we consider,
which implies a maximum fan-in of $2$ and unbounded fan-out 
(that is, the output of a gate might be replicated to many different inputs).
Before proceeding with our main simulation result,
we establish the following useful lemma that we will later use to help tame this standard assumption
of unbounded fan-out. We provide a self-contained proof here. A slightly
smaller constant factor bound can be derived from the technique of Hoover et~al.~\cite{hoover1984bounding}):



\begin{lemma}
Let $Q$ be a circuit with $q$ gates and unbounded fan-out that computes some boolean function $f$.
There exists a circuit $Q'$ with $q' < 3q$ gates that also computes $f$ but has a maximum fan-out of $2$. 
\label{circuit:lem:fan}
\end{lemma}
\begin{proof}
Fix some $Q$ and $f$ as specified by the lemma statement.
Let $G_Q$ be the set of gates in $Q$.
Fix some gate $g\in G_Q$ that connects its output wire to more than two input wires. 
In more detail, let $W_g$ be the set of input wires that connect to $g$'s output.
To connect $g$ to $W_g$ while maintaining a maximum fan-out of $2$ we add some 
additional {\em duplicator} gates that take a single bit as input and duplicate that bit on two output
wires.\footnote{For example, an OR gate with one of the two inputs hard-wired to $0$.}

In more detail, we augment $Q$ to create a binary tree with the input wires in $W_g$ as the leaves,
the output of $g$ the root, and add duplicator gates to play the role of the internal tree nodes.
It is clear that the circuit behavior remains the same as all inputs in $W_g$ receive $g$'s output
in both the original circuit and after our augmentation. 

To account for the extra gates' impact on the circuit size, 
we associate a counter $c[g]$ with each gate $g\in G_Q$, initialized to $1$.
For each augmentation of the type described above, we increment
the gate counters by at least the number of new gates added---ensuring that 
the sum of counters remains an upper bound on the circuit size.

In more detail, for each wire in $W_g$, increment the gate associated with this wire by one.
Because the number of internal nodes in a binary tree is upper bounded by the number of leaves,
the total number of these increments is at least as large as the number of new duplicator gates added
to the circuit during this augmentation step---maintaining our circuit size invariant.

We repeat these augmentations, and accompanying counter increments, until all gates from $G_Q$ with a large fan-out
have had their fan-out reduced to $2$.   Notice, because each gate in in $G_Q$ has at most two input wires,
and each wire can be associated with at most one increment, for every $g' \in G_Q, c[g'] \leq 3$.
It follows at this point that  $\sum_{g' \in G_Q} c[g'] \leq  3|G_Q|$, as required by the lemma.
\end{proof}

\begin{theorem}
Fix some circuit $Q$ that evaluates a boolean function $f:\{0,1\}^n \rightarrow \{0,1\}$.
Assume $Q$ has $cn$ gates for some constant $c> 1$.
There exists a protocol $P_f$ in our model that evaluates $f$ in a network of size $n$
with $lcc(P_f) \leq \lceil 9c \rceil$. 
%such that for every execution $\alpha$ of $P_f$: $ccc(\alpha) \leq \lceil 9c \rceil$.
\label{circuit:thm:sim}
\end{theorem}

\begin{proof}
Fix some $Q$, $f$, and $c$ as specified by the theorem statement.
Let $Q'$ be a circuit with maximum fan-out $2$ and size $q'  < 3cn$ that also computes $f$.
We know such a circuit exists due to Lemma~\ref{circuit:lem:fan}.
Assume without loss of generality that $Q'$ is also optimized in the sense that the output gate is the unique sink in the circuit DAG (i.e.,
there are no {\em wasted} gates whose output has no impact on the output of the circuit).
Finding an efficient procedure for optimizing a circuit in this manner is a hard problem.
But for the purposes, it is sufficient to note that such optimized versions exist.

We now describe the protocol $P_f$  that calculates $f$ in a network of size $n$ by simulating $Q'$.
To do so, we first evenly divide the $q'$ gates among the $n$ nodes in our network.
Each node will be responsible for simulating the no more than the $\lceil 3c \rceil$ gates assigned to it.
We now describe how this simulation behaves and analyze its performance.
For the sake of clarity, we divide the following discussion into parts.

\bigskip

{\em Part $1$: Identify an Activation Ordered Sequence.}
We next order the gates of $Q'$ into a sequence $S_{Q'}$ that satisfy the a useful precedence property.
To do so, we first note that by standard convention each of the $n$ input wires into the circuit are represented in the circuit
by their own gate that has no inputs and a fixed output. 
We call these the {\em input gates}.
%
With this notation fixed, we can define the property we want the sequence $S_{Q'}$ to satisfy:

\begin{quote}
{\em Activation Ordered Property.} The first $n$ gates in $S_{Q'}$ are the $n$ input gates. For every other gate $g$ in $S_{Q'}$,
the gate(s) whose output provides $g$'s inputs come before $g$ in $S_{Q'}$.
\end{quote}

We now provide a constructive proof of the existence of a sequence that satisfies the activation ordered property.
In more detail, we can construct such a sequence with a breadth-first style search through the DAG corresponding to $Q'$.
To do so, we proceed in phases. 
Before the  first phase we initialize our sequence $S_{Q'}$ to contain all $n$ input gates.
We then the following for each phase $i$:

\begin{itemize}
	\item We call a gate $g$ not in $S_{Q'}$ at this point {\em activated} if the gate(s) whose outputs are connected to $g$'s input(s) are in $S_{Q'}$.
	Let $A_i$ be the set of activated gates not in $S_{Q'}$ at this point.
	
	\item If $|S_{Q'}| = 0$ then terminate. Otherwise, append all nodes in $A_i$ to the send of $S_{Q'}$ (in an arbitrary order).
	
	\item If $S_{Q'}$ contains all gates then terminate. Else, repeat the above for the next phase $i+1$.
\end{itemize}

Notice, the above procedure always terminates, and by the fact that it only adds activated gates to the send of the sequence, the sequence produced satisfies the activation ordered property.
The only non-trivial point is proving that this procedure will always produce a sequence that contains all the gates.
To do so, assume for contradiction that it does not; i.e., the $S_{Q'}$ produced does not contain all the gates.
By our above assumption about the optimality of the circuit (no wasted gates that do no influence the output), 
if $S_{Q'}$ is incomplete then it does not contain the output gate.
This sequence, therefore, identifies a functional cut in the circuit DAG across which the computation cannot progress.
This contradicts the assumption that the circuit computes $f$.

\bigskip

{\em Part $2$: Use the Sequence to Schedule the Circuit Simulation.}
Let $S_{Q'}$ be an activation ordered sequence of the type we just proved exist for our circuit. 
We use this sequence to structure protocol $P_f$'s simulation of $Q'$.

In more detail, $S_{Q'}$ passes a token along the nodes simulating the circuit gates in the order specified by $S_{Q'}$.
The token is represented by simply sending a $0$ to the next node in the sequence.
In more detail, the node assigned to simulate the first gate in $S_{Q'}$ sends a $0$ to the node simulating the second gate in $S_{Q'}$.
The node simulating the second gate send a $0$ to the node simulating the third. And so on. If a node is simulating to consecutive nodes
in $S_{Q'}$, it sends itself the token bit.\footnote{This loopback can also be simulated locally, but it is easier to think of it actually sending the message to itself.}

Passing the token provides the structure for the circuit simulation.
To actually execute the computation nodes must also send information about their gates' outputs.
To do so, when a node receives a token on behalf of a gate $g$ that it is simulating,
it calculates the output of $g$, and then ends this bit to the node(s) simulating gate(s) that connect $g$'s output to their input. It does so in a fixed order.
It then sends along the token bit to the next node in the token-passing sequence.

We must be careful here to ensure that the bits received by the simulating nodes (which might correspond to multiple different gates that each node is simulating)
can always be unambiguously interpreted. 
Fortunately, we can leverage the detail in our model definition (Section~\ref{sec:model}) that specifies
that the steps executed along with a scheduled $init$ or $recv$ event, including $send$ commands,
occur atomically at the point the event is scheduled.
Each node can therefore calculate in advance a {\em template} string that describes exactly how many bits it will receive between each token, and to which of its simulated input wires each of these non-token bits correspond to---eliminating any ambiguity about received bits.

In more detail, a given node $u$ simply adds received bits to a local copy of its receive string every time it has a $recv(b)_u$ event scheduled. 
Because it knows its string templates in advance, it knows when a given $recv(0)_u$ event corresponds to the arrival of the token. 
At this point it processes its local copy of the receive string to update the state of the gates it is simulating.
Let $g$ be the simulated gate associated with this token.
By the definition of activation ordered, 
at this point, $u$ has received all inputs for $g$ and has simulated $g$'s output. It can therefore send this bit to the nodes simulating the gates connected to this output,
 and then send on the token bit to the
next node in the order.
It follows that $P_f$ is correctly simulates the gates of $Q'$ in the order they show up in $S_{Q'}$, leading to the output gate correctly determining the output of function $Q'$ at the end of this token passing sequence.

\bigskip 

{\em Step $3$: Calculating the Local Communication Complexity of $P_f$.}
Our final step is to bound the worst case local complexity of $P_f$.
Fix any node $u$.
This node is responsible for simulating at most $\lceil 3c \rceil$ gates.
In the worst case, node $u$ sends and receives a token bit for each of these simulated gates (the total token bits might be less,
as the first gate in $S_{Q'}$ does not require a received token and the last does not require a sent token.)
By assumption, each gate's fan-in is bounded at $2$.
We constructed $Q'$ such that each gate's fan-out is similarly bounded.
It follow that node $u$ has to send at most $2$ output bits and receive at most $2$ input bits for each simulated gate.
Therefore, both $u$'s send and receive complexity is at most  $\lceil 3c \rceil \cdot (1 +2) \leq \lceil 9c\rceil$---as claimed by the theorem statement.
\end{proof}



\noindent The following corollary of Theorem~\ref{circuit:thm:sim} establishes a direct relationship between local complexity
of functions in our model and circuit complexity.


\begin{corollary}
Fix some constant integer $c>9$, network size $n>1$, and boolean function $f:\{0,1\}^n \rightarrow \{0,1\}$
such that $lcc(f) \geq c$.
%
%such that the following is true in our model:
%for every protocol $P$ that computes $f$ in a network of size $n$, $ccc(P) \geq c$.
It follows that every circuit that computes $f$ is of size at least $(c/9)n$.
\label{circuit:corr:sim}
\end{corollary}

\begin{proof}
Fix some $c$, $n$, and $f$ as specified by the corollary statement.
Assume for contradiction that there exists a circuit $C_f$ that computes $f$ and requires $q < (c/9)n$ gates.
By Theorem~\ref{circuit:thm:sim},
there exists a protocol $P_f$ that computes $f$ with a local complexity $x  < \lceil 9(c/9) \rceil = \lceil c \rceil =c$,
where we drop the ceilings in the last step due to the assumption that $c$ is an integer.
Notice, we have just shown a protocol that computes $c$ with a local complexity less than $c$. This contradicts our assumption on the hardness of computing $f$ in our model.
It follows that every circuit that computes $f$ must have a size at least $(c/9)n$, as claimed.  
\end{proof}


This corollary is important because it carries the difficulty of circuit size lower bounds over to our local complexity setting.
The best known circuit complexity lower bounds identify functions that require circuits of size slightly larger than $3n$.
By the above corollary, if we could prove that a given function requires a local complexity slightly larger than $27$,
then we would advance the state of the art in circuit complexity lower bounds, a supremely challenging task.

%The immediate consequence is that we are unlikely to show communication convergence lower bounds beyond certain small constant for specific boolean functions,
%as this would imply strong lower bounds for that function in the circuit complexity setting where such lower bounds are hard.
%For example, if one could show a given function $f$ requires at least some node to send or receive $36$ bits in our model,
%it would follow that all circuits that compute $f$ require at least $4n$ gates---which would be the best known constructive circuit complexity bound ever proved for unrestricted circuits.



\subsection{Simulating Constant Local Complexity Protocols with Linear Size Circuits}
%\subsection{Simulating $C^4$ Protocols with Linear Size Circuits}
%
We now consider the other direction,
and study the simulation of protocols in our model with constant local communication complexity using linear size circuits.
To do so, we (slightly) restrict our attention to {\em value oblivious} protocols (see Section~\ref{sec:model}).
The pre-determined communication structure of value oblivious protocols will allow us to wire a circuit in advance
to handle simulated messages whose content might depend on the circuit inputs.
Multiplexer circuits, each with size exponential in the local complexity, 
are used to select the right simulated outgoing messages depending on the contents of the incoming messages (and relevant input bits).
Because the local complexity is constant, the number of gates required to implement these multiplexers remains constant.
When combined with the preceding theorem,
it follows that there is an equivalence between (value-oblivious) protocols with constant local complexity in our model,
and linear size circuits, in terms of what functions they can compute.

%Formally, we prove the following
%(the proof is deferred to the appendix):

\begin{theorem}
Fix some constant integer $c \geq 1$, network size $n>1$, boolean function $f:\{0,1\}^n \rightarrow \{0,1\}$, and value oblivious protocol $P_f$ 
that computes $f$ with $lcc(P) \leq c$.
It follows that there exists a circuit $C_f$ of size $\Theta(n)$ that computes $f$.
\label{circuit:thm:sim2}
\end{theorem}

\begin{proof}
Fix some $c$, $n$, $f$ and $P_f$ as specified by the theorem statement.
We will identify the required circuit $C_f$ by constructing a circuit that simulates $P_f$ executed with a well-behaved scheduler.

In more detail,
$P_f$ must correctly compute $f$ for all valid schedulers.
One such scheduler is the {\em synchronized scheduler} that behaves as follows:

\begin{enumerate}

	\item Schedule the $init$ events for all $n$ nodes in some fixed order.
	\item Let $S$ be the set of nodes that have non-empty receive strings at this point in the execution.
	Schedule one $recv$ event for each node in $S$ in some fixed order.
	\item If no node has yet output, loop back to step (2).

\end{enumerate}

The synchronized scheduler induces an implicit round structure, where in each round, each node with at least one bit to process, gets to process one bit and execute its corresponding sends. The system
then moves on to the next round.

When this scheduler is combined with a value oblivious protocol like $P_f$,
we can describe the communication of $P$ with a layered DAG $G_P$, where each layer has at most one vertex for each node in the network,
and the links between layers $i$ and $i+1$ correspond to the messages sent in round $i$.
That is, each such directed link $(u,v)$ corresponds to $u$ sending a message $v$ during round $i$.
Because $P_f$ is value oblivious, this same DAG describes the communication structure for every execution with the synchronized scheduler.
The only thing that potentially changes between different input assignments are the specific bits contained in the messages sent on those predetermined links.\footnote{A subtle point
in constructing $G_P$ is that we also rely on the assumption that value oblivious protocols must send messages of the same {\em size} for a given destination
and round. This assumption is part of the definition of value oblivious given in Section~\ref{sec:model}. 
This size requirement is needed to construct $G_P$ as otherwise a node's receive string might be empty at different points in the execution
depending on the input values in the system.}
Notice, as an obvious optimization, we do not include a vertex corresponding to node $u$ in layer $i$ if $u$ does not send or receive messages in that layer. 

We now construct a circuit $C_f$ that simulates $P_f$ executed with a synchronous scheduler.
To do so, we setup the circuit that matches the structure of $G_P$.
Each layer $i+1$ vertex in $G_P$ is implemented with a multiplexer that takes as input the bits of the messages received from its neighbors from layer $i$,
and outputs to its neighbors in layer $i+2$ the bits of the messages that correspond to the specific pattern it received in $i$.

Implementing such a multiplexer can require a number of gates exponential in the number of input and output wires.
We assumed, however, that $P_f$ has a local complexity no more than $c=\Theta(1)$.
It follows that none of our multiplexers require more than $c$ incoming or outgoing wires, allowing
us to bound the size of each multiplexer's implementation by some $c'$ that is exponential in $c$.
Because $c$ is constant, so is $c'$.

The resulting circuit size is now $c' |V_P|$ (plus some overhead for the input and output gates), which
is in $\Theta(|V_P|)$, where $V_P$ is the set of vertices in $G_P$.
Each node can show up at most $2c$ times in $G_P$ layers, as otherwise it would violate the local complexity bound of $c$.
It follows that $|V_P| \leq 2cn = \Theta(n)$ and therefore $C_f$'s total size is linear in $n$---as required by the theorem statement.
\end{proof}


\iffalse
\subsection{Value Oblivious Versus Adaptive}
%\label{sec:oblivious}
%
Our protocol simulation result worked only for {\em value oblivious} protocols.
A relevant follow-up question is whether the value oblivious constraint is necessary, or if, perhaps, there instead exists 
a way to transform any adaptive protocol to an equivalent protocol in a
value oblivious form (making this assumption hold without loss of generality).
In Appendix~\ref{app:oblivious}, we prove no such general transformation exists
by defining a novel function that can be solved with an adaptive protocol with minimum local complexity of $1$, but that, as we prove,
cannot be computed with this same local complexity by a value oblivious strategy.
In addition to providing the claimed separation, the novel argument used to prove this impossibility is
of standalone interest as it represents only the second known constructive lower bound in the local complexity setting.

\fi
